Scalable, Advanced Machine Learning-based Approaches for Stellar Flare Identification: Application to TESS short-cadence Data and Analysis of a New Flare Catalogue

We apply multi-algorithm machine learning models to TESS 2-minute survey data from Sectors 1-72 to identify stellar flares. Models trained with Deep Neural Network, Random Forest, and XGBoost algorithms, respectively, utilized four flare light curve characteristics as input features. Model performance is evaluated using accuracy, precision, recall, and F1-score metrics, all exceeding 94%. Validation against previously reported TESS M dwarf flare identifications showed that our models successfully recovered over 92% of the flares while detecting $\sim2,000$ more small events, thus extending the detection sensitivity of previous work. After processing 1.3 million light curves, our models identified nearly 18,000 flare stars and 250,000 flares. We present an extensive catalog documenting both flare and stellar properties. We find strong correlations in total flare energy and flare amplitude with color, in agreement with previous studies. Flare frequency distributions are analyzed, refining power-law slopes for flare behavior with the frequency uncertainties due to the detection incompleteness of low-amplitude events. We determine rotation periods for $\sim120,000$ stars thus yielding the relationship between rotation period and flare activity. We find that the transition in rotation period between the saturated and unsaturated regimes in flare energy coincides with the same transition in rotation period separating the saturated and unsaturated levels in coronal X-ray emission. We find that X-ray emission increases more rapidly with flare luminosity in earlier-type and unsaturated stars, indicating more efficient coronal heating in these objects. Additionally, we detect flares in white dwarfs and hot subdwarfs that are likely arising from unresolved low-mass companions.

==> manuscript_bibtex.tex <==
\clearpage
\begin{thebibliography}{}

\bibitem{2018AJ....156..123A}Astropy Collaboration, Price-Whelan, A., Sipőcz, B., Günther, H., Lim, P., Crawford, S., Conseil, S., Shupe, D., Craig, M., Dencheva, N., Ginsburg, A., VanderPlas, J., Bradley, L., Pérez-Suárez, D., De Val-Borro, M., Aldcroft, T., Cruz, K., Robitaille, T., Tollerud, E., Ardelean, C., Babej, T., Bach, Y., Bachetti, M., Bakanov, A., Bamford, S., Barentsen, G., Barmby, P., Baumbach, A., Berry, K., Biscani, F., Boquien, M., Bostroem, K., Bouma, L., Brammer, G., Bray, E., Breytenbach, H., Buddelmeijer, H., Burke, D., Calderone, G., Cano Rodrı́guez, J., Cara, M., Cardoso, J., Cheedella, S., Copin, Y., Corrales, L., Crichton, D., D'Avella, D., Deil, C., Depagne, É., Dietrich, J., Donath, A., Droettboom, M., Earl, N., Erben, T., Fabbro, S., Ferreira, L., Finethy, T., Fox, R., Garrison, L., Gibbons, S., Goldstein, D., Gommers, R., Greco, J., Greenfield, P., Groener, A., Grollier, F., Hagen, A., Hirst, P., Homeier, D., Horton, A., Hosseinzadeh, G., Hu, L., Hunkeler, J., Ivezić, Ž., Jain, A., Jenness, T., Kanarek, G., Kendrew, S., Kern, N., Kerzendorf, W., Khvalko, A., King, J., Kirkby, D., Kulkarni, A., Kumar, A., Lee, A., Lenz, D., Littlefair, S., Ma, Z., Macleod, D., Mastropietro, M., McCully, C., Montagnac, S., Morris, B., Mueller, M., Mumford, S., Muna, D., Murphy, N., Nelson, S., Nguyen, G., Ninan, J., Nöthe, M., Ogaz, S., Oh, S., Parejko, J., Parley, N., Pascual, S., Patil, R., Patil, A., Plunkett, A., Prochaska, J., Rastogi, T., Reddy Janga, V., Sabater, J., Sakurikar, P., Seifert, M., Sherbert, L., Sherwood-Taylor, H., Shih, A., Sick, J., Silbiger, M., Singanamalla, S., Singer, L., Sladen, P., Sooley, K., Sornarajah, S., Streicher, O., Teuben, P., Thomas, S., Tremblay, G., Turner, J., Terrón, V., Van Kerkwijk, M., De la Vega, A., Watkins, L., Weaver, B., Whitmore, J., Woillez, J., Zabalza, V. \& Astropy Contributors The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package. {\em \aj}. \textbf{156}, e123 (2018,9)
\bibitem{breiman1996bagging}Breiman, L. Bagging predictors. {\em Machine Learning}. \textbf{24} pp. 123-140 (1996)
\bibitem{2015A&A...581A..28P}Pye, J., Rosen, S., Fyfe, D. \& Schröder, A. A survey of stellar X-ray flares from the XMM-Newton serendipitous source catalogue: HIPPARCOS-Tycho cool stars. {\em \aap}. \textbf{581} pp. eA28 (2015,9)
\bibitem{2022ApJ...927..179T}Toriumi, S. \& Airapetian, V. Universal Scaling Laws for Solar and Stellar Atmospheric Heating. {\em \apj}. \textbf{927}, e179 (2022,3)
\bibitem{2005ApJ...621..398O}Osten, R., Hawley, S., Allred, J., Johns-Krull, C. \& Roark, C. From Radio to X-Ray: Flares on the dMe Flare Star EV Lacertae. {\em \apj}. \textbf{621}, 398-416 (2005,3)
\bibitem{2019ApJ...871..167K}Kowalski, A., Wisniewski, J., Hawley, S., Osten, R., Brown, A., Fariña, C., Valenti, J., Brown, S., Xilouris, M., Schmidt, S. \& Johns-Krull, C. The Near-ultraviolet Continuum Radiation in the Impulsive Phase of HF/GF-type dMe Flares. I. Data. {\em \apj}. \textbf{871}, e167 (2019,2)
\bibitem{2009A&A...496..577Z}Zechmeister, M. \& Kürster, M. The generalised Lomb-Scargle periodogram. A new formalism for the floating-mean and Keplerian periodograms. {\em \aap}. \textbf{496}, 577-584 (2009,3)
\bibitem{2014ApJ...797..121H}Hawley, S., Davenport, J., Kowalski, A., Wisniewski, J., Hebb, L., Deitrick, R. \& Hilton, E. Kepler Flares. I. Active and Inactive M Dwarfs. {\em \apj}. \textbf{797}, e121 (2014,12)
\bibitem{2015ApJ...798...92W}Wu, C., Ip, W. \& Huang, L. A Study of Variability in the Frequency Distributions of the Superflares of G-type Stars Observed by the Kepler Mission. {\em \apj}. \textbf{798}, e92 (2015,1)
\bibitem{2018ApJ...867...78C}Chang, H., Lin, C., Ip, W., Huang, L., Hou, W., Yu, P., Song, Y. \& Luo, A. Hyperflares of M Dwarfs. {\em \apj}. \textbf{867}, e78 (2018,11)
\bibitem{2020ApJ...905..110B}Bai, J. \& Esamdin, A. Flare Properties of A-type Stars in Kepler Data. {\em \apj}. \textbf{905}, e110 (2020,12)
\bibitem{2009SIAMR..51..661C}Clauset, A., Shalizi, C. \& Newman, M. Power-Law Distributions in Empirical Data. {\em SIAM Review}. \textbf{51}, 661-703 (2009,1)
\bibitem{2023A+A...669A..15Y}Yang, Z., Zhang, L., Meng, G., Han, X., Misra, P., Yang, J. \& Pi, Q. Properties of flare events based on light curves from the TESS survey. {\em \aap}. \textbf{669} pp. eA15 (2023,1)
\bibitem{2010AsBio..10..751S}Segura, A., Walkowicz, L., Meadows, V., Kasting, J. \& Hawley, S. The Effect of a Strong Stellar Flare on the Atmospheric Chemistry of an Earth-like Planet Orbiting an M Dwarf. {\em Astrobiology}. \textbf{10}, 751-771 (2010,9)
\bibitem{2024MNRAS.527.8290P}Petrucci, R., Gómez Maqueo Chew, Y., Jofré, E., Segura, A. \& Ferrero, L. Exploring the photometric variability of ultra-cool dwarfs with TESS. {\em \mnras}. \textbf{527}, 8290-8304 (2024,1)
\bibitem{1963ApJS....8..177P}Parker, E. The Solar-Flare Phenomenon and the Theory of Reconnection and Annihiliation of Magnetic Fields.. {\em \apjs}. \textbf{8} pp. 177 (1963,7)
\bibitem{2015ApJ...809...77S}Sullivan, P., Winn, J., Berta-Thompson, Z., Charbonneau, D., Deming, D., Dressing, C., Latham, D., Levine, A., McCullough, P., Morton, T., Ricker, G., Vanderspek, R. \& Woods, D. The Transiting Exoplanet Survey Satellite: Simulations of Planet Detections and Astrophysical False Positives. {\em \apj}. \textbf{809}, e77 (2015,8)
\bibitem{2021arXiv210804778P}Paegert, M., Stassun, K., Collins, K., Pepper, J., Torres, G., Jenkins, J., Twicken, J. \& Latham, D. TESS Input Catalog versions 8.1 and 8.2: Phantoms in the 8.0 Catalog and How to Handle Them. {\em ArXiv E-prints}. pp. earXiv:2108.04778 (2021,8)
\bibitem{2017SoPh..292...77G}Gryciuk, M., Siarkowski, M., Sylwester, J., Gburek, S., Podgorski, P., Kepa, A., Sylwester, B. \& Mrozek, T. Flare Characteristics from X-ray Light Curves. {\em \solphys}. \textbf{292}, e77 (2017,6)
\bibitem{2020pase.conf..226B}Barron, J., Wade, G., Bowman, D., David-Uraz, A., Munoz, M., Pablo, H. \& Simón-Dı́z, S. MOBSTER: Identifying Candidate Magnetic O Stars through Rotational Modulation of TESS Photometry. {\em Stellar Magnetism: A Workshop In Honour Of The Career And Contributions Of John D. Landstreet}. \textbf{11} pp. 226-235 (2020,11)
\bibitem{1972ApJ...171..565S}Skumanich, A. Time Scales for Ca II Emission Decay, Rotational Braking, and Lithium Depletion. {\em \apj}. \textbf{171} pp. 565 (1972,2)
\bibitem{2012Natur.485..478M}Maehara, H., Shibayama, T., Notsu, S., Notsu, Y., Nagao, T., Kusaba, S., Honda, S., Nogami, D. \& Shibata, K. Superflares on solar-type stars. {\em \nat}. \textbf{485}, 478-481 (2012,5)
\bibitem{2019ApJ...871..241D}Davenport, J., Covey, K., Clarke, R., Boeck, A., Cornet, J. \& Hawley, S. The Evolution of Flare Activity with Stellar Age. {\em \apj}. \textbf{871}, e241 (2019,2)
\bibitem{2011ApJ...743...48W}Wright, N., Drake, J., Mamajek, E. \& Henry, G. The Stellar-activity-Rotation Relationship and the Evolution of Stellar Dynamos. {\em \apj}. \textbf{743}, e48 (2011,12)
\bibitem{2003A&A...397..147P}Pizzolato, N., Maggio, A., Micela, G., Sciortino, S. \& Ventura, P. The stellar activity-rotation relationship revisited: Dependence of saturated and non-saturated X-ray emission regimes on stellar mass for late-type dwarfs. {\em \aap}. \textbf{397} pp. 147-157 (2003,1)
\bibitem{2019A&A...628A..41P}Pizzocaro, D., Stelzer, B., Poretti, E., Raetz, S., Micela, G., Belfiore, A., Marelli, M., Salvetti, D. \& De Luca, A. Activity and rotation of the X-ray emitting Kepler stars. {\em \aap}. \textbf{628} pp. eA41 (2019,8)
\bibitem{2009ApJ...692..538R}Reiners, A., Basri, G. \& Browning, M. Evidence for Magnetic Flux Saturation in Rapidly Rotating M Stars. {\em \apj}. \textbf{692}, 538-545 (2009,2)
\bibitem{2016SPIE.9913E..3EJ}Jenkins, J., Twicken, J., McCauliff, S., Campbell, J., Sanderfer, D., Lung, D., Mansouri-Samani, M., Girouard, F., Tenenbaum, P., Klaus, T., Smith, J., Caldwell, D., Chacon, A., Henze, C., Heiges, C., Latham, D., Morgan, E., Swade, D., Rinehart, S. \& Vanderspek, R. The TESS science processing operations center. {\em Software And Cyberinfrastructure For Astronomy IV}. \textbf{9913} pp. e99133E (2016,8)
\bibitem{2018arXiv180308375A}Agarap, A. Deep Learning using Rectified Linear Units (ReLU). {\em ArXiv E-prints}. pp. earXiv:1803.08375 (2018,3)
\bibitem{2019ApJ...873...97L}Lin, C., Ip, W., Hou, W., Huang, L. \& Chang, H. A Comparative Study of the Magnetic Activities of Low-mass Stars from M-type to G-type. {\em \apj}. \textbf{873}, e97 (2019,3)
\bibitem{2021MNRAS.504.3246J}Jackman, J., Wheatley, P., Acton, J., Anderson, D., Bayliss, D., Briegal, J., Burleigh, M., Casewell, S., Gänsicke, B., Gill, S., Gillen, E., Goad, M., Günther, M., Henderson, B., Hodgkin, S., Jenkins, J., Pugh, C., Queloz, D., Raynard, L., Tilbrook, R., Watson, C. \& West, R. Stellar flares detected with the Next Generation Transit Survey. {\em \mnras}. \textbf{504}, 3246-3264 (2021,7)
\bibitem{2000ApJ...529.1026S}Schaefer, B., King, J. \& Deliyannis, C. Superflares on Ordinary Solar-Type Stars. {\em \apj}. \textbf{529}, 1026-1030 (2000,2)
\bibitem{2023MNRAS.519.3564J}Jackman, J., Shkolnik, E., Million, C., Fleming, S., Richey-Yowell, T. \& Loyd, R. Extending optical flare models to the UV: results from comparing of TESS and GALEX flare observations for M Dwarfs. {\em \mnras}. \textbf{519}, 3564-3583 (2023,3)
\bibitem{2021ApJ...910...41A}Aschwanden, M. \& Güdel, M. Self-organized Criticality in Stellar Flares. {\em \apj}. \textbf{910}, e41 (2021,3)
\bibitem{2022yCat..22580016P}Prsa, A., Kochoska, A., Conroy, K., Eisner, N., Hey, D., Ijspeert, L., Kruse, E., Fleming, S., Johnston, C., Kristiansen, M., Lacourse, D., Mortensen, D., Pepper, J., Stassun, K., Torres, G., Abdul-Masih, M., Chakraborty, J., Gagliano, R., Guo, Z., Hambleton, K., Hong, K., Jacobs, T., Jones, D., Kostov, V., Lee, J., Omohundro, M., Orosz, J., Page, E., Powell, B., Rappaport, S., Reed, P., Schnittman, J., Schwengeler, H., Shporer, A., Terentev, I., Vanderburg, A., Welsh, W., Caldwell, D., Doty, J., Jenkins, J., Latham, D., Ricker, G., Seager, S., Schlieder, J., Shiao, B., Vanderspek, R. \& Winn, J. VizieR Online Data Catalog: TESS Eclipsing Binary stars. I. Sectors 1-26 (Prsa+, 2022). {\em VizieR Online Data Catalog}. pp. eJ/ApJS/258/16 (2022,8)
\bibitem{1976Ap&SS..39..447L}Lomb, N. Least-Squares Frequency Analysis of Unequally Spaced Data. {\em \apss}. \textbf{39}, 447-462 (1976,2)
\bibitem{1982ApJ...263..835S}Scargle, J. Studies in astronomical time series analysis. II. Statistical aspects of spectral analysis of unevenly spaced data.. {\em \apj}. \textbf{263} pp. 835-853 (1982,12)
\bibitem{2020A&A...637A..22R}Raetz, S., Stelzer, B., Damasso, M. \& Scholz, A. Rotation-activity relations and flares of M dwarfs with K2 long- and short-cadence data. {\em \aap}. \textbf{637} pp. eA22 (2020,5)
\bibitem{NIPS1989_0336dcba}Bridle, J. Training Stochastic Model Recognition Algorithms as Networks can Lead to Maximum Mutual Information Estimation of Parameters. {\em Advances In Neural Information Processing Systems}. \textbf{2} (1989), https://proceedings.neurips.cc/paper_files/paper/1989/file/0336dcbab05b9d5ad24f4333c7658a0e-Paper.pdf
\bibitem{chawla2002smote}Chawla, N., Bowyer, K., Hall, L. \& Kegelmeyer, W. SMOTE: synthetic minority over-sampling technique. {\em Journal Of Artificial Intelligence Research}. \textbf{16} pp. 321-357 (2002)
\bibitem{JMLR:v18:16-365}Lemaître, G., Nogueira, F. \& Aridas, C. Imbalanced-learn: A Python Toolbox to Tackle the Curse of Imbalanced Datasets in Machine Learning. {\em Journal Of Machine Learning Research}. \textbf{18}, 1-5 (2017), http://jmlr.org/papers/v18/16-365
\bibitem{2018ascl.soft12013L}Lightkurve Collaboration, Cardoso, J., Hedges, C., Gully-Santiago, M., Saunders, N., Cody, A., Barclay, T., Hall, O., Sagear, S., Turtelboom, E., Zhang, J., Tzanidakis, A., Mighell, K., Coughlin, J., Bell, K., Berta-Thompson, Z., Williams, P., Dotson, J. \& Barentsen, G. Lightkurve: Kepler and TESS time series analysis in Python. (Astrophysics Source Code Library, record ascl:1812.013,2018,12)
\bibitem{2013A&A...558A..33A}Astropy Collaboration, Robitaille, T., Tollerud, E., Greenfield, P., Droettboom, M., Bray, E., Aldcroft, T., Davis, M., Ginsburg, A., Price-Whelan, A., Kerzendorf, W., Conley, A., Crighton, N., Barbary, K., Muna, D., Ferguson, H., Grollier, F., Parikh, M., Nair, P., Unther, H., Deil, C., Woillez, J., Conseil, S., Kramer, R., Turner, J., Singer, L., Fox, R., Weaver, B., Zabalza, V., Edwards, Z., Azalee Bostroem, K., Burke, D., Casey, A., Crawford, S., Dencheva, N., Ely, J., Jenness, T., Labrie, K., Lim, P., Pierfederici, F., Pontzen, A., Ptak, A., Refsdal, B., Servillat, M. \& Streicher, O. Astropy: A community Python package for astronomy. {\em \aap}. \textbf{558} pp. eA33 (2013,10)
\bibitem{1996A&AS..117..393B}Bertin, E. \& Arnouts, S. SExtractor: Software for source extraction.. {\em \aaps}. \textbf{117} pp. 393-404 (1996,6)
\bibitem{2018AJ....156...82C}Cloutier, R., Doyon, R., Bouchy, F. \& Hébrard, G. Quantifying the Observational Effort Required for the Radial Velocity Characterization of TESS Planets. {\em \aj}. \textbf{156}, e82 (2018,8)
\bibitem{2015ApJ...805...23C}Corrales, L. X-Ray Scattering Echoes and Ghost Halos from the Intergalactic Medium: Relation to the Nature of AGN Variability. {\em \apj}. \textbf{805}, e23 (2015,5)
\bibitem{2013RMxAA..49..137F}Ferland, G., Porter, R., Van Hoof, P., Williams, R., Abel, N., Lykins, M., Shaw, G., Henney, W. \& Stancil, P. The 2013 Release of Cloudy. {\em \rmxaa}. \textbf{49} pp. 137-163 (2013,4)
\bibitem{1989BAAS...21..780H}Hanisch, R. \& Biemesderfer, C. T<sub>E</sub>X and LAT<sub>E</sub>X Macro Definition Files for Astronomical Publications. {\em \baas}. pp. 780 (1989,3)
\bibitem{lamport94}Lamport, L. LaTeX: A Document Preparation System. (Addison-Wesley Professional,1994)
\bibitem{2018ApJ...868L..33L}Li, L., Zhang, J., Peter, H., Chitta, L., Su, J., Song, H., Xia, C. \& Hou, Y. Quasi-periodic Fast Propagating Magnetoacoustic Waves during the Magnetic Reconnection Between Solar Coronal Loops. {\em \apj}. \textbf{868}, eL33 (2018,12)
\bibitem{2016AJ....152...41P}Prša, A., Harmanec, P., Torres, G., Mamajek, E., Asplund, M., Capitaine, N., Christensen-Dalsgaard, J., Depagne, É., Haberreiter, M. \& Hekker, S. Nominal Values for Selected Solar and Planetary Quantities: IAU 2015 Resolution B3. {\em \aj}. \textbf{152}, e41 (2016,8)
\bibitem{2015ApJ...814...35C}Chang, S., Byun, Y. \& Hartman, J. Photometric Study on Stellar Magnetic Activity. I. Flare Variability of Red Dwarf Stars in the Open Cluster M37. {\em \apj}. \textbf{814}, e35 (2015,11)
\bibitem{1999A&AS..139..555G}Gershberg, R., Katsova, M., Lovkaya, M., Terebizh, A. \& Shakhovskaya, N. Catalogue and bibliography of the UV Cet-type flare stars and related objects in the solar vicinity. {\em \aaps}. \textbf{139} pp. 555-558 (1999,11)
\bibitem{2020ApJ...905..107M}Medina, A., Winters, J., Irwin, J. \& Charbonneau, D. Flare Rates, Rotation Periods, and Spectroscopic Activity Indicators of a Volume-complete Sample of Mid- to Late-M Dwarfs within 15 pc. {\em \apj}. \textbf{905}, e107 (2020,12)
\bibitem{2017ApJ...834...92C}Chang, H., Song, Y., Luo, A., Huang, L., Ip, W., Fu, J., Zhang, Y., Hou, Y., Cao, Z. \& Wang, Y. LAMOST Observations of Flaring M Dwarfs in the Kepler Field. {\em \apj}. \textbf{834}, e92 (2017,1)
\bibitem{2017MNRAS.468.1946H}Hermes, J., Gänsicke, B., Gentile Fusillo, N., Raddi, R., Hollands, M., Dennihy, E., Fuchs, J. \& Redfield, S. When flux standards go wild: white dwarfs in the age of Kepler. {\em \mnras}. \textbf{468}, 1946-1952 (2017,6)
\bibitem{2021ApJ...914L...3H}Hermes, J., Putterman, O., Hollands, M., Wilson, D., Swan, A., Raddi, R., Shen, K. \& Gänsicke, B. 8.9 hr Rotation in the Partly Burnt Runaway Stellar Remnant LP 40-365 (GD 492). {\em \apjl}. \textbf{914}, eL3 (2021,6)
\bibitem{2022MNRAS.515.2496P}Pelisoli, I., Dorsch, M., Heber, U., Gänsicke, B., Geier, S., Kupfer, T., Németh, P., Scaringi, S. \& Schaffenroth, V. Discovery and analysis of three magnetic hot subdwarf stars: evidence for merger-induced magnetic fields. {\em \mnras}. \textbf{515}, 2496-2510 (2022,9)
\bibitem{2007ApJ...669.1167B}Barnes, S. Ages for Illustrative Field Stars Using Gyrochronology: Viability, Limitations, and Errors. {\em \apj}. \textbf{669}, 1167-1189 (2007,11)
\bibitem{2007CSE.....9...90H}Hunter, J. Matplotlib: A 2D Graphics Environment. {\em Computing In Science And Engineering}. \textbf{9}, 90-95 (2007,5)
\bibitem{harris2020array}Harris, C., Millman, K., Walt, S., Gommers, R., Virtanen, P., Cournapeau, D., Wieser, E., Taylor, J., Berg, S., Smith, N., Kern, R., Picus, M., Hoyer, S., Kerkwijk, M., Brett, M., Haldane, A., Río, J., Wiebe, M., Peterson, P., Gérard-Marchant, P., Sheppard, K., Reddy, T., Weckesser, W., Abbasi, H., Gohlke, C. \& Oliphant, T. Array programming with NumPy. {\em Nature}. \textbf{585}, 357-362 (2020,9), https://doi.org/10.1038/s41586-020-2649-2
\bibitem{mckinney2010data}McKinney, W. \& Others Data structures for statistical computing in python. {\em Proceedings Of The 9th Python In Science Conference}. \textbf{445} pp. 51-56 (2010)
\bibitem{https://doi.org/10.17909/t9-nmc8-f686}Team, M. TESS Light Curves - All Sectors. (STScI/MAST,2021), http://archive.stsci.edu/doi/resolve/resolve.html?doi=10.17909/t9-nmc8-f686
\bibitem{2018AJ....156..178Z}Zhang, Z., Zhou, Y., Rackham, B. \& Apai, D. The Near-infrared Transmission Spectra of TRAPPIST-1 Planets b, c, d, e, f, and g and Stellar Contamination in Multi-epoch Transit Spectra. {\em \aj}. \textbf{156}, e178 (2018,10)
\bibitem{goodfellow2016deep}Goodfellow, I., Bengio, Y. \& Courville, A. Deep learning. (MIT press,2016)
\bibitem{2023AJ....166...82L}Lin, C., Ip, W., Hsiao, Y., Chang, T., Song, Y. \& Luo, A. Mass Accretion, Spectral, and Photometric Properties of T Tauri Stars in Taurus Based on TESS and LAMOST. {\em \aj}. \textbf{166}, e82 (2023,9)
\bibitem{2023ASPC..534..355F}Fischer, W., Hillenbrand, L., Herczeg, G., Johnstone, D., Kospal, A. \& Dunham, M. Accretion Variability as a Guide to Stellar Mass Assembly. {\em Protostars And Planets VII}. \textbf{534} pp. 355 (2023,7)
\bibitem{2021PASP..133c4503H}Huang, C., Lehner, M., Granados Contreras, A., Castro-Chacón, J., Chen, W., Alcock, C., Alvarez-Santana, F., Cook, K., Geary, J., Guerrero Peña, C., Hernández-Águila, J., Hernández-Valencia, B., Karr, J., Kavelaars, J., Norton, T., Nuñez, J., Ochoa, D., Reyes-Ruiz, M., Sánchez, E., Silva, J., Szentgyorgyi, A., Wang, S., Yen, W. \& Zhang, Z. The TAOS II Survey: Real-time Detection and Characterization of Occultation Events. {\em \pasp}. \textbf{133}, e034503 (2021,3)
\bibitem{2022arXiv220606693G}Ge, J., Zhang, H., Zang, W., Deng, H., Mao, S., Xie, J., Liu, H., Zhou, J., Willis, K., Huang, C., Howell, S., Feng, F., Zhu, J., Yao, X., Liu, B., Aizawa, M., Zhu, W., Li, Y., Ma, B., Ye, Q., Yu, J., Xiang, M., Yu, C., Liu, S., Yang, M., Wang, M., Shi, X., Fang, T., Zong, W., Liu, J., Zhang, Y., Zhang, L., El-Badry, K., Shen, R., Tam, P., Hu, Z., Yang, Y., Zou, Y., Wu, J., Lei, W., Wei, J., Wu, X., Sun, T., Wang, F., Zhang, B., Xu, D., Yang, Y., Li, W., Xiang, D., Wang, X., Wang, T., Zhang, B., Jia, P., Yuan, H., Zhang, J., Xuesong Wang, S., Gan, T., Wang, W., Zhao, Y., Liu, Y., Wei, C., Kang, Y., Yang, B., Qi, C., Liu, X., Zhang, Q., Zhu, Y., Zhou, D., Zhang, C., Yu, Y., Zhang, Y., Li, Y., Tang, Z., Wang, C., Wang, F., Li, W., Cheng, P., Shen, C., Li, B., Pan, Y., Yang, S., Gao, W., Song, Z., Wang, J., Zhang, H., Chen, C., Wang, H., Zhang, J., Wang, Z., Zeng, F., Zheng, Z., Zhu, J., Guo, Y., Zhang, Y., Li, Y., Wen, L., Feng, J., Chen, W., Chen, K., Han, X., Yang, Y., Wang, H., Duan, X., Huang, J., Liang, H., Bi, S., Gai, N., Ge, Z., Guo, Z., Huang, Y., Li, G., Li, H., Li, T., Yuxi, Lu, Rix, H., Shi, J., Song, F., Tang, Y., Ting, Y., Wu, T., Wu, Y., Yang, T., Yin, Q., Gould, A., Lee, C., Dong, S., Yee, J., Shvartzvald, Y., Yang, H., Kuang, R., Zhang, J., Liao, S., Qi, Z., Yang, J., Zhang, R., Jiang, C., Ou, J., Li, Y., Beck, P., Bedding, T., Campante, T., Chaplin, W., Christensen-Dalsgaard, J., Garcı́a, R., Gaulme, P., Gizon, L., Hekker, S., Huber, D., Khanna, S., Li, Y., Mathur, S., Miglio, A., Mosser, B., Ong, J., Santos, Â., Stello, D., Bowman, D., Lares-Martiz, M., Murphy, S., Niu, J., Ma, X., Molnár, L., Fu, J., De Cat, P., Su, J. \& Consortium, T. ET White Paper: To Find the First Earth 2.0. {\em ArXiv E-prints}. pp. earXiv:2206.06693 (2022,6)
\bibitem{2014ExA....38..249R}Rauer, H., Catala, C., Aerts, C., Appourchaux, T., Benz, W., Brandeker, A., Christensen-Dalsgaard, J., Deleuil, M., Gizon, L., Goupil, M., Güdel, M., Janot-Pacheco, E., Mas-Hesse, M., Pagano, I., Piotto, G., Pollacco, D., Santos, Ċ., Smith, A., Suárez, J., Szabó, R., Udry, S., Adibekyan, V., Alibert, Y., Almenara, J., Amaro-Seoane, P., Eiff, M., Asplund, M., Antonello, E., Barnes, S., Baudin, F., Belkacem, K., Bergemann, M., Bihain, G., Birch, A., Bonfils, X., Boisse, I., Bonomo, A., Borsa, F., Brandão, I., Brocato, E., Brun, S., Burleigh, M., Burston, R., Cabrera, J., Cassisi, S., Chaplin, W., Charpinet, S., Chiappini, C., Church, R., Csizmadia, S., Cunha, M., Damasso, M., Davies, M., Deeg, H., Dı́az, R., Dreizler, S., Dreyer, C., Eggenberger, P., Ehrenreich, D., Eigmüller, P., Erikson, A., Farmer, R., Feltzing, S., De Oliveira Fialho, F., Figueira, P., Forveille, T., Fridlund, M., Garcı́a, R., Giommi, P., Giuffrida, G., Godolt, M., Gomes da Silva, J., Granzer, T., Grenfell, J., Grotsch-Noels, A., Günther, E., Haswell, C., Hatzes, A., Hébrard, G., Hekker, S., Helled, R., Heng, K., Jenkins, J., Johansen, A., Khodachenko, M., Kislyakova, K., Kley, W., Kolb, U., Krivova, N., Kupka, F., Lammer, H., Lanza, A., Lebreton, Y., Magrin, D., Marcos-Arenal, P., Marrese, P., Marques, J., Martins, J., Mathis, S., Mathur, S., Messina, S., Miglio, A., Montalban, J., Montalto, M., Monteiro, M., Moradi, H., Moravveji, E., Mordasini, C., Morel, T., Mortier, A., Nascimbeni, V., Nelson, R., Nielsen, M., Noack, L., Norton, A., Ofir, A., Oshagh, M., Ouazzani, R., Pápics, P., Parro, V., Petit, P., Plez, B., Poretti, E., Quirrenbach, A., Ragazzoni, R., Raimondo, G., Rainer, M., Reese, D., Redmer, R., Reffert, S., Rojas-Ayala, B., Roxburgh, I., Salmon, S., Santerne, A., Schneider, J., Schou, J., Schuh, S., Schunker, H., Silva-Valio, A., Silvotti, R., Skillen, I., Snellen, I., Sohl, F., Sousa, S., Sozzetti, A., Stello, D., Strassmeier, K., Švanda, M., Szabó, G., Tkachenko, A., Valencia, D., Van Grootel, V., Vauclair, S., Ventura, P., Wagner, F., Walton, N., Weingrill, J., Werner, S., Wheatley, P. \& Zwintz, K. The PLATO 2.0 mission. {\em Experimental Astronomy}. \textbf{38}, 249-330 (2014,11)
\bibitem{2015arXiv150303757S}Spergel, D., Gehrels, N., Baltay, C., Bennett, D., Breckinridge, J., Donahue, M., Dressler, A., Gaudi, B., Greene, T., Guyon, O., Hirata, C., Kalirai, J., Kasdin, N., Macintosh, B., Moos, W., Perlmutter, S., Postman, M., Rauscher, B., Rhodes, J., Wang, Y., Weinberg, D., Benford, D., Hudson, M., Jeong, W., Mellier, Y., Traub, W., Yamada, T., Capak, P., Colbert, J., Masters, D., Penny, M., Savransky, D., Stern, D., Zimmerman, N., Barry, R., Bartusek, L., Carpenter, K., Cheng, E., Content, D., Dekens, F., Demers, R., Grady, K., Jackson, C., Kuan, G., Kruk, J., Melton, M., Nemati, B., Parvin, B., Poberezhskiy, I., Peddie, C., Ruffa, J., Wallace, J., Whipple, A., Wollack, E. \& Zhao, F. Wide-Field InfrarRed Survey Telescope-Astrophysics Focused Telescope Assets WFIRST-AFTA 2015 Report. {\em ArXiv E-prints}. pp. earXiv:1503.03757 (2015,3)
\bibitem{2016MNRAS.457.3988B}Boyajian, T., LaCourse, D., Rappaport, S., Fabrycky, D., Fischer, D., Gandolfi, D., Kennedy, G., Korhonen, H., Liu, M., Moor, A., Olah, K., Vida, K., Wyatt, M., Best, W., Brewer, J., Ciesla, F., Csák, B., Deeg, H., Dupuy, T., Handler, G., Heng, K., Howell, S., Ishikawa, S., Kovács, J., Kozakis, T., Kriskovics, L., Lehtinen, J., Lintott, C., Lynn, S., Nespral, D., Nikbakhsh, S., Schawinski, K., Schmitt, J., Smith, A., Szabo, G., Szabo, R., Viuho, J., Wang, J., Weiksnar, A., Bosch, M., Connors, J., Goodman, S., Green, G., Hoekstra, A., Jebson, T., Jek, K., Omohundro, M., Schwengeler, H. \& Szewczyk, A. Planet Hunters IX. KIC 8462852 - where's the flux?. {\em \mnras}. \textbf{457}, 3988-4004 (2016,4)
\bibitem{2015JATIS...1a4003R}Ricker, G., Winn, J., Vanderspek, R., Latham, D., Bakos, G., Bean, J., Berta-Thompson, Z., Brown, T., Buchhave, L., Butler, N., Butler, R., Chaplin, W., Charbonneau, D., Christensen-Dalsgaard, J., Clampin, M., Deming, D., Doty, J., De Lee, N., Dressing, C., Dunham, E., Endl, M., Fressin, F., Ge, J., Henning, T., Holman, M., Howard, A., Ida, S., Jenkins, J., Jernigan, G., Johnson, J., Kaltenegger, L., Kawai, N., Kjeldsen, H., Laughlin, G., Levine, A., Lin, D., Lissauer, J., MacQueen, P., Marcy, G., McCullough, P., Morton, T., Narita, N., Paegert, M., Palle, E., Pepe, F., Pepper, J., Quirrenbach, A., Rinehart, S., Sasselov, D., Sato, B., Seager, S., Sozzetti, A., Stassun, K., Sullivan, P., Szentgyorgyi, A., Torres, G., Udry, S. \& Villasenor, J. Transiting Exoplanet Survey Satellite (TESS). {\em Journal Of Astronomical Telescopes, Instruments, And Systems}. \textbf{1} pp. e014003 (2015,1)
\bibitem{tensorflow2015-whitepaper}Abadi, M., Agarwal, A., Barham, P., Brevdo, E., Chen, Z., Citro, C., Corrado, G., Davis, A., Dean, J., Devin, M., Ghemawat, S., Goodfellow, I., Harp, A., Irving, G., Isard, M., Jia, Y., Jozefowicz, R., Kaiser, L., Kudlur, M., Levenberg, J., Mané, D., Monga, R., Moore, S., Murray, D., Olah, C., Schuster, M., Shlens, J., Steiner, B., Sutskever, I., Talwar, K., Tucker, P., Vanhoucke, V., Vasudevan, V., Viégas, F., Vinyals, O., Warden, P., Wattenberg, M., Wicke, M., Yu, Y. \& Zheng, X.  TensorFlow: Large-Scale Machine Learning on Heterogeneous Systems.  (2015), https://www.tensorflow.org/, Software available from tensorflow.org
\bibitem{2020NatMe..17..261V}Virtanen, P., Gommers, R., Oliphant, T., Haberland, M., Reddy, T., Cournapeau, D., Burovski, E., Peterson, P., Weckesser, W., Bright, J., Van der Walt, S., Brett, M., Wilson, J., Millman, K., Mayorov, N., Nelson, A., Jones, E., Kern, R., Larson, E., Carey, C., Polat, İ., Feng, Y., Moore, E., VanderPlas, J., Laxalde, D., Perktold, J., Cimrman, R., Henriksen, I., Quintero, E., Harris, C., Archibald, A., Ribeiro, A., Pedregosa, F., Van Mulbregt, P. \& SciPy 1. 0 Contributors SciPy 1.0: fundamental algorithms for scientific computing in Python. {\em Nature Methods}. \textbf{17} pp. 261-272 (2020,2)
\bibitem{2022ApJ...935..167A}Astropy Collaboration, Price-Whelan, A., Lim, P., Earl, N., Starkman, N., Bradley, L., Shupe, D., Patil, A., Corrales, L., Brasseur, C., Nöthe, M., Donath, A., Tollerud, E., Morris, B., Ginsburg, A., Vaher, E., Weaver, B., Tocknell, J., Jamieson, W., Van Kerkwijk, M., Robitaille, T., Merry, B., Bachetti, M., Günther, H., Aldcroft, T., Alvarado-Montes, J., Archibald, A., Bódi, A., Bapat, S., Barentsen, G., Bazán, J., Biswas, M., Boquien, M., Burke, D., Cara, D., Cara, M., Conroy, K., Conseil, S., Craig, M., Cross, R., Cruz, K., D'Eugenio, F., Dencheva, N., Devillepoix, H., Dietrich, J., Eigenbrot, A., Erben, T., Ferreira, L., Foreman-Mackey, D., Fox, R., Freij, N., Garg, S., Geda, R., Glattly, L., Gondhalekar, Y., Gordon, K., Grant, D., Greenfield, P., Groener, A., Guest, S., Gurovich, S., Handberg, R., Hart, A., Hatfield-Dodds, Z., Homeier, D., Hosseinzadeh, G., Jenness, T., Jones, C., Joseph, P., Kalmbach, J., Karamehmetoglu, E., Kałuszyński, M., Kelley, M., Kern, N., Kerzendorf, W., Koch, E., Kulumani, S., Lee, A., Ly, C., Ma, Z., MacBride, C., Maljaars, J., Muna, D., Murphy, N., Norman, H., O'Steen, R., Oman, K., Pacifici, C., Pascual, S., Pascual-Granado, J., Patil, R., Perren, G., Pickering, T., Rastogi, T., Roulston, B., Ryan, D., Rykoff, E., Sabater, J., Sakurikar, P., Salgado, J., Sanghi, A., Saunders, N., Savchenko, V., Schwardt, L., Seifert-Eckert, M., Shih, A., Jain, A., Shukla, G., Sick, J., Simpson, C., Singanamalla, S., Singer, L., Singhal, J., Sinha, M., Sipőcz, B., Spitler, L., Stansby, D., Streicher, O., Šumak, J., Swinbank, J., Taranu, D., Tewary, N., Tremblay, G., De Val-Borro, M., Van Kooten, S., Vasović, Z., Verma, S., De Miranda Cardoso, J., Williams, P., Wilson, T., Winkel, B., Wood-Vasey, W., Xue, R., Yoachim, P., Zhang, C., Zonca, A. \& Astropy Project Contributors The Astropy Project: Sustaining and Growing a Community-oriented Open-source Project and the Latest Major Release (v5.0) of the Core Package. {\em \apj}. \textbf{935}, e167 (2022,8)
\bibitem{2020AJ....159...60G}Günther, M., Zhan, Z., Seager, S., Rimmer, P., Ranjan, S., Stassun, K., Oelkers, R., Daylan, T., Newton, E., Kristiansen, M., Olah, K., Gillen, E., Rappaport, S., Ricker, G., Vanderspek, R., Latham, D., Winn, J., Jenkins, J., Glidden, A., Fausnaugh, M., Levine, A., Dittmann, J., Quinn, S., Krishnamurthy, A. \& Ting, E. Stellar Flares from the First TESS Data Release: Exploring a New Sample of M Dwarfs. {\em \aj}. \textbf{159}, e60 (2020,2)
\bibitem{scikit-learn}Pedregosa, F., Varoquaux, G., Gramfort, A., Michel, V., Thirion, B., Grisel, O., Blondel, M., Prettenhofer, P., Weiss, R., Dubourg, V., Vanderplas, J., Passos, A., Cournapeau, D., Brucher, M., Perrot, M. \& Duchesnay, E. Scikit-learn: Machine Learning in Python. {\em Journal Of Machine Learning Research}. \textbf{12} pp. 2825-2830 (2011)
\bibitem{breiman2001random}Breiman, L. Random forests. {\em Machine Learning}. \textbf{45} pp. 5-32 (2001)
\bibitem{chen2016xgboost}Chen, T. \& Guestrin, C. Xgboost: A scalable tree boosting system. {\em Proceedings Of The 22nd Acm Sigkdd International Conference On Knowledge Discovery And Data Mining}. pp. 785-794 (2016)
\bibitem{51791361-8fe2-38d5-959f-ae8d048b490d}Tibshirani, R. Regression Shrinkage and Selection via the Lasso. {\em Journal Of The Royal Statistical Society. Series B (Methodological)}. \textbf{58}, 267-288 (1996), http://www.jstor.org/stable/2346178
\bibitem{a92f3c16-7c6e-31d3-b403-82d2b0a469e4}Hoerl, A. \& Kennard, R. Ridge Regression: Biased Estimation for Nonorthogonal Problems. {\em Technometrics}. \textbf{12}, 55-67 (1970), http://www.jstor.org/stable/1267351
\bibitem{sklearn_api}Buitinck, L., Louppe, G., Blondel, M., Pedregosa, F., Mueller, A., Grisel, O., Niculae, V., Prettenhofer, P., Gramfort, A., Grobler, J., Layton, R., VanderPlas, J., Joly, A., Holt, B. \& Varoquaux, G. API design for machine learning software: experiences from the scikit-learn project. {\em ECML PKDD Workshop: Languages For Data Mining And Machine Learning}. pp. 108-122 (2013)
\bibitem{geron2022hands}Géron, A. Hands-on machine learning with Scikit-Learn, Keras, and TensorFlow. (" O'Reilly Media, Inc.",2022)
\bibitem{chollet2015keras}Chollet, F. \& Others Keras. (GitHub,2015), https://github.com/fchollet/keras
\bibitem{1972Ap&SS..19...75G}Gershberg, R. Some results of the cooperative photometric observations of the UV Cet-type flare stars in the years 1967 71. {\em \apss}. \textbf{19}, 75-92 (1972,11)
\bibitem{8694781}Shrestha, A. \& Mahmood, A. Review of Deep Learning Algorithms and Architectures. {\em IEEE Access}. \textbf{7} pp. 53040-53065 (2019)
\bibitem{2014arXiv1412.6980K}Kingma, D. \& Ba, J. Adam: A Method for Stochastic Optimization. {\em ArXiv E-prints}. pp. earXiv:1412.6980 (2014,12)
\bibitem{2019arXiv190407248B}Baron, D. Machine Learning in Astronomy: a practical overview. {\em ArXiv E-prints}. pp. earXiv:1904.07248 (2019,4)
\bibitem{2015Natur.521..436L}LeCun, Y., Bengio, Y. \& Hinton, G. Deep learning. {\em \nat}. \textbf{521}, 436-444 (2015,5)
\bibitem{2021NatAs...5..298C}Chen, H., Zhan, Z., Youngblood, A., Wolf, E., Feinstein, A. \& Horton, D. Persistence of flare-driven atmospheric chemistry on rocky habitable zone worlds. {\em Nature Astronomy}. \textbf{5} pp. 298-310 (2021,1)
\bibitem{2022ApJ...926..204H}Howard, W. \& MacGregor, M. No Such Thing as a Simple Flare: Substructure and Quasi-periodic Pulsations Observed in a Statistical Sample of 20 s Cadence TESS Flares. {\em \apj}. \textbf{926}, e204 (2022,2)
\bibitem{2021AJ....162...11L}Lin, C., Chen, W., Ip, W., Apai, D., Bixel, A., Boyle, R., Chavez, J., Espinoza, N., Gibbs, A., Gabor, P., Henning, T., Mancini, L., Rackham, B., Schlecker, M., Dietrich, J., Socia, Q., Keppler, M., Bhandare, A. \& Häberle, M. EDEN: Flare Activity of the Nearby Exoplanet-hosting M Dwarf Wolf 359 Based on K2 and EDEN Light Curves. {\em \aj}. \textbf{162}, e11 (2021,7)
\bibitem{2018ApJ...853..122R}Rackham, B., Apai, D. \& Giampapa, M. The Transit Light Source Effect: False Spectral Features and Incorrect Densities for M-dwarf Transiting Planets. {\em \apj}. \textbf{853}, e122 (2018,2)
\bibitem{2023AJ....165..149D}Dietrich, J., Apai, D., Schlecker, M., Hardegree-Ullman, K., Rackham, B., Kurtovic, N., Molaverdikhani, K., Gabor, P., Henning, T., Chen, W., Mancini, L., Bixel, A., Gibbs, A., Boyle, R., Brown-Sevilla, S., Burn, R., Delage, T., Flores-Rivera, L., Franceschi, R., Pichierri, G., Savvidou, S., Syed, J., Bruni, I., Ip, W., Ngeow, C., Tsai, A., Lin, C., Hou, W., Hsiao, H., Lin, C., Lin, H., Basant, R. \& EDEN Project EDEN Survey: Small Transiting Planet Detection Limits and Constraints on the Occurrence Rates of Planets around Late-M Dwarfs within 15 pc. {\em \aj}. \textbf{165}, e149 (2023,4)
\bibitem{2023ApJ...959...64H}Howard, W., Kowalski, A., Flagg, L., MacGregor, M., Lim, O., Radica, M., Piaulet, C., Roy, P., Lafrenière, D., Benneke, B., Brown, A., Espinoza, N., Doyon, R., Coulombe, L., Johnstone, D., Cowan, N., Jayawardhana, R., Turner, J. \& Dang, L. Characterizing the Near-infrared Spectra of Flares from TRAPPIST-1 during JWST Transit Spectroscopy Observations. {\em \apj}. \textbf{959}, e64 (2023,12)
\bibitem{2013ApJS..209....5S}Shibayama, T., Maehara, H., Notsu, S., Notsu, Y., Nagao, T., Honda, S., Ishii, T., Nogami, D. \& Shibata, K. Superflares on Solar-type Stars Observed with Kepler. I. Statistical Properties of Superflares. {\em \apjs}. \textbf{209}, e5 (2013,11)
\bibitem{2014MNRAS.445.2268P}Pitkin, M., Williams, D., Fletcher, L. \& Grant, S. A Bayesian method for detecting stellar flares. {\em \mnras}. \textbf{445}, 2268-2284 (2014,12)
\bibitem{2021MNRAS.506.5681D}Dal Tio, P., Mazzi, A., Girardi, L., Barbieri, M., Zaggia, S., Bressan, A., Chen, Y., Costa, G. \& Marigo, P. Dissecting the Gaia HR diagram within 200 pc. {\em \mnras}. \textbf{506}, 5681-5697 (2021,10)
\bibitem{2021ApJS..253...35T}Tu, Z., Yang, M., Wang, H. \& Wang, F. Superflares, Chromospheric Activities, and Photometric Variabilities of Solar-type Stars from the Second-year Observation of TESS and Spectra of LAMOST. {\em \apjs}. \textbf{253}, e35 (2021,4)
\bibitem{2022A&A...664A.105F}Freund, S., Czesla, S., Robrade, J., Schneider, P. \& Schmitt, J. The stellar content of the ROSAT all-sky survey. {\em \aap}. \textbf{664} pp. eA105 (2022,8)
\bibitem{2024ApJS..271...57X}Xing, K., Zong, W., Silvotti, R., Fu, J., Charpinet, S., Cang, T., Hermes, J., Ma, X., Wang, H., Wang, X., Wu, T. \& Wang, J. Flare Hunting in Hot Subdwarf and White Dwarf Stars from Cycles 1–5 of TESS Photometry. {\em \apjs}. \textbf{271}, e57 (2024,4)
\bibitem{2019AJ....158..138S}Stassun, K., Oelkers, R., Paegert, M., Torres, G., Pepper, J., De Lee, N., Collins, K., Latham, D., Muirhead, P., Chittidi, J., Rojas-Ayala, B., Fleming, S., Rose, M., Tenenbaum, P., Ting, E., Kane, S., Barclay, T., Bean, J., Brassuer, C., Charbonneau, D., Ge, J., Lissauer, J., Mann, A., McLean, B., Mullally, S., Narita, N., Plavchan, P., Ricker, G., Sasselov, D., Seager, S., Sharma, S., Shiao, B., Sozzetti, A., Stello, D., Vanderspek, R., Wallace, G. \& Winn, J. The Revised TESS Input Catalog and Candidate Target List. {\em \aj}. \textbf{158}, e138 (2019,10)
\bibitem{2023A&A...674A...1G}Gaia Collaboration, Vallenari, A., Brown, A., Prusti, T., De Bruijne, J., Arenou, F., Babusiaux, C., Biermann, M., Creevey, O., Ducourant, C., Evans, D., Eyer, L., Guerra, R., Hutton, A., Jordi, C., Klioner, S., Lammers, U., Lindegren, L., Luri, X., Mignard, F., Panem, C., Pourbaix, D., Randich, S., Sartoretti, P., Soubiran, C., Tanga, P., Walton, N., Bailer-Jones, C., Bastian, U., Drimmel, R., Jansen, F., Katz, D., Lattanzi, M., Van Leeuwen, F., Bakker, J., Cacciari, C., Castañeda, J., De Angeli, F., Fabricius, C., Fouesneau, M., Frémat, Y., Galluccio, L., Guerrier, A., Heiter, U., Masana, E., Messineo, R., Mowlavi, N., Nicolas, C., Nienartowicz, K., Pailler, F., Panuzzo, P., Riclet, F., Roux, W., Seabroke, G., Sordo, R., Thévenin, F., Gracia-Abril, G., Portell, J., Teyssier, D., Altmann, M., Andrae, R., Audard, M., Bellas-Velidis, I., Benson, K., Berthier, J., Blomme, R., Burgess, P., Busonero, D., Busso, G., Cánovas, H., Carry, B., Cellino, A., Cheek, N., Clementini, G., Damerdji, Y., Davidson, M., De Teodoro, P., Nuñez Campos, M., Delchambre, L., Dell'Oro, A., Esquej, P., Fernández-Hernández, J., Fraile, E., Garabato, D., Garcı́a-Lario, P., Gosset, E., Haigron, R., Halbwachs, J., Hambly, N., Harrison, D., Hernández, J., Hestroffer, D., Hodgkin, S., Holl, B., Janßen, K., Jevardat de Fombelle, G., Jordan, S., Krone-Martins, A., Lanzafame, A., Löffler, W., Marchal, O., Marrese, P., Moitinho, A., Muinonen, K., Osborne, P., Pancino, E., Pauwels, T., Recio-Blanco, A., Reylé, C., Riello, M., Rimoldini, L., Roegiers, T., Rybizki, J., Sarro, L., Siopis, C., Smith, M., Sozzetti, A., Utrilla, E., Van Leeuwen, M., Abbas, U., Ábrahám, P., Abreu Aramburu, A., Aerts, C., Aguado, J., Ajaj, M., Aldea-Montero, F., Altavilla, G., Álvarez, M., Alves, J., Anders, F., Anderson, R., Anglada Varela, E., Antoja, T., Baines, D., Baker, S., Balaguer-Núñez, L., Balbinot, E., Balog, Z., Barache, C., Barbato, D., Barros, M., Barstow, M., Bartolomé, S., Bassilana, J., Bauchet, N., Becciani, U., Bellazzini, M., Berihuete, A., Bernet, M., Bertone, S., Bianchi, L., Binnenfeld, A., Blanco-Cuaresma, S., Blazere, A., Boch, T., Bombrun, A., Bossini, D., Bouquillon, S., Bragaglia, A., Bramante, L., Breedt, E., Bressan, A., Brouillet, N., Brugaletta, E., Bucciarelli, B., Burlacu, A., Butkevich, A., Buzzi, R., Caffau, E., Cancelliere, R., Cantat-Gaudin, T., Carballo, R., Carlucci, T., Carnerero, M., Carrasco, J., Casamiquela, L., Castellani, M., Castro-Ginard, A., Chaoul, L., Charlot, P., Chemin, L., Chiaramida, V., Chiavassa, A., Chornay, N., Comoretto, G., Contursi, G., Cooper, W., Cornez, T., Cowell, S., Crifo, F., Cropper, M., Crosta, M., Crowley, C., Dafonte, C., Dapergolas, A., David, M., David, P., De Laverny, P., De Luise, F., De March, R., De Ridder, J., De Souza, R., De Torres, A., Del Peloso, E., Del Pozo, E., Delbo, M., Delgado, A., Delisle, J., Demouchy, C., Dharmawardena, T., Di Matteo, P., Diakite, S., Diener, C., Distefano, E., Dolding, C., Edvardsson, B., Enke, H., Fabre, C., Fabrizio, M., Faigler, S., Fedorets, G., Fernique, P., Fienga, A., Figueras, F., Fournier, Y., Fouron, C., Fragkoudi, F., Gai, M., Garcia-Gutierrez, A., Garcia-Reinaldos, M., Garcı́a-Torres, M., Garofalo, A., Gavel, A., Gavras, P., Gerlach, E., Geyer, R., Giacobbe, P., Gilmore, G., Girona, S., Giuffrida, G., Gomel, R., Gomez, A., González-Núñez, J., González-Santamarı́a, I., González-Vidal, J., Granvik, M., Guillout, P., Guiraud, J., Gutiérrez-Sánchez, R., Guy, L., Hatzidimitriou, D., Hauser, M., Haywood, M., Helmer, A., Helmi, A., Sarmiento, M., Hidalgo, S., Hilger, T., Hładczuk, N., Hobbs, D., Holland, G., Huckle, H., Jardine, K., Jasniewicz, G., Jean-Antoine Piccolo, A., Jiménez-Arranz, Ó., Jorissen, A., Juaristi Campillo, J., Julbe, F., Karbevska, L., Kervella, P., Khanna, S., Kontizas, M., Kordopatis, G., Korn, A., Kóspál, Á., Kostrzewa-Rutkowska, Z., Kruszyńska, K., Kun, M., Laizeau, P., Lambert, S., Lanza, A., Lasne, Y., Le Campion, J., Lebreton, Y., Lebzelter, T., Leccia, S., Leclerc, N., Lecoeur-Taibi, I., Liao, S., Licata, E., Lindstrøm, H., Lister, T., Livanou, E., Lobel, A., Lorca, A., Loup, C., Madrero Pardo, P., Magdaleno Romeo, A., Managau, S., Mann, R., Manteiga, M., Marchant, J., Marconi, M., Marcos, J., Marcos Santos, M., Marı́n Pina, D., Marinoni, S., Marocco, F., Marshall, D., Martin Polo, L., Martı́n-Fleitas, J., Marton, G., Mary, N., Masip, A., Massari, D., Mastrobuono-Battisti, A., Mazeh, T., McMillan, P., Messina, S., Michalik, D., Millar, N., Mints, A., Molina, D., Molinaro, R., Molnár, L., Monari, G., Monguió, M., Montegriffo, P., Montero, A., Mor, R., Mora, A., Morbidelli, R., Morel, T., Morris, D., Muraveva, T., Murphy, C., Musella, I., Nagy, Z., Noval, L., Ocaña, F., Ogden, A., Ordenovic, C., Osinde, J., Pagani, C., Pagano, I., Palaversa, L., Palicio, P., Pallas-Quintela, L., Panahi, A., Payne-Wardenaar, S., Peñalosa Esteller, X., Penttilä, A., Pichon, B., Piersimoni, A., Pineau, F., Plachy, E., Plum, G., Poggio, E., Prša, A., Pulone, L., Racero, E., Ragaini, S., Rainer, M., Raiteri, C., Rambaux, N., Ramos, P., Ramos-Lerate, M., Re Fiorentin, P., Regibo, S., Richards, P., Rios Diaz, C., Ripepi, V., Riva, A., Rix, H., Rixon, G., Robichon, N., Robin, A., Robin, C., Roelens, M., Rogues, H., Rohrbasser, L., Romero-Gómez, M., Rowell, N., Royer, F., Ruz Mieres, D., Rybicki, K., Sadowski, G., Sáez Núñez, A., Sagristà Sellés, A., Sahlmann, J., Salguero, E., Samaras, N., Sanchez Gimenez, V., Sanna, N., Santoveña, R., Sarasso, M., Schultheis, M., Sciacca, E., Segol, M., Segovia, J., Ségransan, D., Semeux, D., Shahaf, S., Siddiqui, H., Siebert, A., Siltala, L., Silvelo, A., Slezak, E., Slezak, I., Smart, R., Snaith, O., Solano, E., Solitro, F., Souami, D., Souchay, J., Spagna, A., Spina, L., Spoto, F., Steele, I., Steidelmüller, H., Stephenson, C., Süveges, M., Surdej, J., Szabados, L., Szegedi-Elek, E., Taris, F., Taylor, M., Teixeira, R., Tolomei, L., Tonello, N., Torra, F., Torra, J., Torralba Elipe, G., Trabucchi, M., Tsounis, A., Turon, C., Ulla, A., Unger, N., Vaillant, M., Van Dillen, E., Van Reeven, W., Vanel, O., Vecchiato, A., Viala, Y., Vicente, D., Voutsinas, S., Weiler, M., Wevers, T., Wyrzykowski, Ł., Yoldas, A., Yvard, P., Zhao, H., Zorec, J., Zucker, S. \& Zwitter, T. Gaia Data Release 3. Summary of the content and survey properties. {\em \aap}. \textbf{674} pp. eA1 (2023,6)
\bibitem{2022AJ....163..147G}Gilbert, E., Barclay, T., Quintana, E., Walkowicz, L., Vega, L., Schlieder, J., Monsue, T., Cale, B., Collins, K., Gaidos, E., El Mufti, M., Reefe, M., Plavchan, P., Tanner, A., Wittenmyer, R., Wittrock, J., Jenkins, J., Latham, D., Ricker, G., Rose, M., Seager, S., Vanderspek, R. \& Winn, J. Flares, Rotation, and Planets of the AU Mic System from TESS Observations. {\em \aj}. \textbf{163}, e147 (2022,4)
\bibitem{2018A&A...616A.163V}Vida, K. \& Roettenbacher, R. Finding flares in Kepler data using machine-learning tools. {\em \aap}. \textbf{616} pp. eA163 (2018,9)
\bibitem{2021A&A...652A.107V}Vida, K., Bódi, A., Szklenár, T. \& Seli, B. Finding flares in Kepler and TESS data with recurrent deep neural networks. {\em \aap}. \textbf{652} pp. eA107 (2021,8)
\bibitem{2022ApJ...935...90T}Tu, Z., Wu, Q., Wang, W., Zhang, G., Liu, Z. \& Wang, F. Convolutional Neural Networks for Searching Superflares from Pixel-level Data of the Transiting Exoplanet Survey Satellite. {\em \apj}. \textbf{935}, e90 (2022,8)
\bibitem{2020AJ....160..219F}Feinstein, A., Montet, B., Ansdell, M., Nord, B., Bean, J., Günther, M., Gully-Santiago, M. \& Schlieder, J. Flare Statistics for Young Stars from a Convolutional Neural Network Analysis of TESS Data. {\em \aj}. \textbf{160}, e219 (2020,11)
\bibitem{2012MNRAS.423.3420B}Balona, L. Kepler observations of flaring in A-F type stars. {\em \mnras}. \textbf{423}, 3420-3429 (2012,7)
\bibitem{2016ApJ...829...23D}Davenport, J. The Kepler Catalog of Stellar Flares. {\em \apj}. \textbf{829}, e23 (2016,9)
\bibitem{2019ApJS..241...29Y}Yang, H. \& Liu, J. The Flare Catalog and the Flare Activity in the Kepler Mission. {\em \apjs}. \textbf{241}, e29 (2019,4)
\bibitem{2019ApJ...884..160V}Vida, K., Oláh, K., Kővári, Z., Van Driel-Gesztelyi, L., Moór, A. \& Pál, A. Flaring Activity of Proxima Centauri from TESS Observations: Quasiperiodic Oscillations during Flare Decay and Inferences on the Habitability of Proxima b. {\em \apj}. \textbf{884}, e160 (2019,10)
\bibitem{2011ApJS..197...31S}Schwarz, G., Ness, J., Osborne, J., Page, K., Evans, P., Beardmore, A., Walter, F., Helton, L., Woodward, C., Bode, M., Starrfield, S. \& Drake, J. Swift X-Ray Observations of Classical Novae. II. The Super Soft Source Sample. {\em \apjs}. \textbf{197}, e31 (2011,12)
\bibitem{2014ApJ...793..127V}Vogt, F., Dopita, M., Kewley, L., Sutherland, R., Scharwächter, J., Basurah, H., Ali, A. \& Amer, M. Galaxy Emission Line Classification Using Three-dimensional Line Ratio Diagrams. {\em \apj}. \textbf{793}, e127 (2014,10)


\end{thebibliography}
